Energy-aware Time- and Event-triggered KVM Nodes

Industries are considering the adoption of cloud and edge computing for real-time applications due to current improvements in network latencies and the advent of Fog and Edge computing. Current cloud paradigms are not designed for real-time applications, as they neither provide low latencies/jitter nor the guarantees and determinism required by real-time applications. Experts estimate that data centers use 1% of global electricity for powering the equipment, and in turn, for dealing with the produced heat. Hence, energy consumption is a crucial metric in cloud technologies. Applying energy conservation techniques is not straightforward due to the increased scheduling overheads and application execution times. Inspired by slot shifting, we propose an algorithm to support energy-aware time-triggered execution of periodic real-time VMs while still providing the ability to execute aperiodic real-time and best-effort VMs in the slack of the time-triggered ones. The algorithm considers energy reduction techniques based on dynamic power management and dynamic voltage and frequency scaling. We implement our algorithm as an extension to the Linux kernel scheduler (for use with the KVM hypervisor) and evaluate it on a server-grade Intel Xeon node.

==> Section_How_To.tex <==





\section{How to Use Commenting in this Document}

This document supports commenting. The main styles for comments are included in "comment.tex" file. 
There are 6 types of comments:
\begin{itemize}
	\item \textbf{Main Comment}: Green comments are used to show main comment about some part of the text. 
	Name of the person appears in the beginning of the comment if that person is already defined in "comments.tex" file. 
	We usually use combination of the first name and last name. 
	For example, "mn" stands for Mitra Nasri. 
	Thus, \textit{mncomment} command appears with name "Mitra".
	Example: \gfcomment{Sample comment by Gerhard.}  \mncomment{Sample comment by Mitra.} 
	
	\item \textbf{Anonymous Comment}: For anonymous comment, or for those who are not in the "comments.tex" file, it is possible to use \textit{comment} command. Example: \comment{Anonymous comment.}
	
	\item \textbf{Main Reply}: It is used to show that the following message is a reply to a comment. 
	Example: 
	\mnreply{Sample replay comment by Mitra Nasri. } 
	\\
	\reply{Anonymous reply.}
	
	\item \textbf{Figure is Missing Comment}: This comment shows a figure is missing. 
	Example: 
	\mnfiguremissing{Here we need Figure 2.}
	
	\item \textbf{Side Comment}: Side comments appear close to the text, and not as a part of text. For these comments, write as minimum words as possible. 
	They make the document ugly, but they are easy to trace. 
	Example: 
	\mnsidecomment{Test}
	\textbf{Note:} If you use this comment, you need to compile the document 3 times to get your correct comment right. ;-)
	
	\item \textbf{Outline Comment}: All previous comments are inline. 
	If you want to show itemized lists use outlines. 
	Outlines are not assigned to people's names. 
	Example:
	\outline{ Here we have an outline. 
	\begin{itemize}
		\item It can have several items.
		\item It accepts many types of formatting.
		\item It highlights the concerns.
		\item It is very useful for structuring the text. 
	\end{itemize}
	}

\end{itemize}

















==> Suffix.tex <==



%-------------------------------------------------------------------%


%\section*{Acknowledgment}
%The work presented in this paper has been supported by the German Academic Exchange Service (DAAD) scholarship. 



\bibliographystyle{IEEEtran}      % basic style, author-year citations
\bibliography{References}   % name your BibTeX data base


\end{document}





% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation Results}
%\label{fig_sim}
%\end{figure}

% Note that IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command, the
% \label for the overall figure must come after \caption.
% \hfil must be used as a separator to get equal spacing.
% The subfigure.sty package works much the same way, except \subfigure is
% used instead of \subfloat.
%
%\begin{figure*}[!t]
%\centerline{\subfloat[Case I]\includegraphics[width=2.5in]{subfigcase1}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{subfigcase2}%
%\label{fig_second_case}}}
%\caption{Simulation results}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.


% An example of a floating table. Note that, for IEEE style tables, the 
% \caption command should come BEFORE the table. Table text will default to
% \footnotesize as IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
%\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
%\caption{An Example of a Table}
%\label{table_example}
%\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
%\begin{tabular}{|c||c|}
%\hline
%One & Two\\
%\hline
%Three & Four\\
%\hline
%\end{tabular}
%\end{table}


% Note that IEEE does not put floats in the very first column - or typically
% anywhere on the first page for that matter. Also, in-text middle ("here")
% positioning is not used. Most IEEE journals/conferences use top floats
% exclusively. Note that, LaTeX2e, unlike IEEE journals/conferences, places
% footnotes above bottom floats. This can be corrected via the \fnbelowfloat
% command of the stfloats package.

